Improving the Learning of Code Review Successive Tasks with Cross-Task Knowledge Distillation

Code review is a fundamental process in software development that plays a pivotal role in ensuring code quality and reducing the likelihood of errors and bugs. However, code review can be complex, subjective, and time-consuming. Quality estimation, comment generation, and code refinement constitute the three key tasks of this process, and their automation has traditionally been addressed separately in the literature using different approaches. In particular, recent efforts have focused on fine-tuning pre-trained language models to aid in code review tasks, with each task being considered in isolation. We believe that these tasks are interconnected, and their fine-tuning should consider this interconnection. In this paper, we introduce a novel deep-learning architecture, named DISCOREV, which employs cross-task knowledge distillation to address these tasks simultaneously. In our approach, we utilize a cascade of models to enhance both comment generation and code refinement models. The fine-tuning of the comment generation model is guided by the code refinement model, while the fine-tuning of the code refinement model is guided by the quality estimation model. We implement this guidance using two strategies: a feedback-based learning objective and an embedding alignment objective. We evaluate DISCOREV by comparing it to state-of-the-art methods based on independent training and fine-tuning. Our results show that our approach generates better review comments, as measured by the BLEU score, as well as more accurate code refinement according to the CodeBLEU score

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections/2-background-backup.tex <==
\section{Background}
\label{sec:background}


\subsection{Code review}
\label{Sec:code_review}
In a continuous integration setting, software developers utilize version control systems, such as GitHub, to collaborate and oversee software versions. 
As developers collaborate and persistently make changes to the codebase (\ie write new code or modify existing code), the use of version control systems enables development teams to efficiently manage and monitor the software codebase across time  \cite{shahin2017continuous, fowler2006continuous}. 
\Fig{fig:pr1} illustrates the conventional software development workflow in a continuous integration context.



% \begin{figure}[h]
%   \centering
%   \includegraphics[width=1\linewidth]{figures/pull-request-bw2.png}
%   \caption{Conventional software development workflow in a continuous integration context}
%   \label{fig:pr1}
% \end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{figures/pull-request-color.png}
  \caption{Conventional software development workflow in a continuous integration context}
  \label{fig:pr1}
\end{figure}


A developer, who is working on implementing a new feature, makes local changes to the codebase.
Then, she commits and pushes her changes to a shared repository \circled{1} to make the new changes available to collaborators.
She can create a pull request \circled{2} to request that her changes be merged to the main branch (\ie main version of the source code). 
Some reviewers are assigned to the pull request \circled{3} to inspect the code changes made by the author before these changes are merged with the main branch. 
Reviewers identify and locate issues \circled{4} that need to be solved by the code author (\circled{5} and \circled{6}). 
The revised version of the code, submitted by developers, should be reviewed again.
Once these changes are approved by reviewers, they are merged with the main code version, \ie main branch \circled{7}, to be available to other developers (\ie collaborators).
If necessary, the project can be deployed \circled{8}, so that changes will be available to end-users.


% Code review

Code review is an essential task in the software development life cycle that aims to preserve the high quality of the software's codebase.
It entails regularly inspecting the source code written by fellow developers with the objective of identifying bugs, potential issues, sub-optimal code fragments, violations of code style, etc.
\Fig{fig:crprocess} depicts an overview of this process.



\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{figures/codereview-process-2.png}
  \caption{Process of code review}
  \label{fig:crprocess}
\end{figure}


The process of code review is triggered once a developer pushes her code to a remote shared repository.
The developer creates a pull request, \ie asks to merge her changes with the main codebase to make them available.
Prior to the merge with the main branch, these changes need to be inspected by going through a code review process.
The first step of this process involves assigning one or more reviewers to the pull request \circled{A}. This phase depends on many factors including expertise, availability, etc.
If the code is well-written and does not have problems \circled{B}, the pull request is accepted and the code changes are merged with the main branch of the codebase.
Conversely, if the code has issues, the reviewer should identify them \circled{C}.
She writes a comment to describe the issues at hand \circled{D} and potentially suggests some solutions.
Subsequently, the developer should address the comment by fixing the issues and applying the appropriate corrections\circled{E}. 
This is a recurring process where the developer should push the new changes to be checked again by the reviewers. 
If the issues are properly fixed, the reviewer accepts the pull request.
Otherwise, she could give further explanations or point out newly introduced issues.



\paragraph*{\textbf{Quality estimation}}
The nomenclature \emph{quality estimation} is adopted herein, in harmony with the work elucidated in \cite{li2022automating}, to maintain terminological consistency.
It is a pivotal step of the code review process that represents the assessment of a pull request, ultimately culminating in the consequential decision of either acceptance or rejection. 
It's the process of carefully looking at the changes someone wants to make to the code and deciding if those changes are good enough to be added to the project or if they need some improvements.
During this process, the reviewer checks the code to ensure it follows the rules, works correctly, and won't cause problems in the project. Quality estimation helps maintain the overall quality of the software by only accepting changes that meet certain criteria.
If the pull request is accepted, the code changes are merged with the main branch of the codebase. Otherwise, the reviewer needs to explain the problems or the required improvements that the developer should consider. After making the necessary changes by the developer, the new code changes go through the process of quality estimation again.


\paragraph*{\textbf{Code review comments}}
Having assigned a reviewer to the pull request, her role is to inspect the newly introduced changes to the codebase. The reviewer examines the source code changes looking for issues or potential improvements. Issues might be related to security vulnerabilities, code style, code standards violations, inconsistencies, bugs, sub-optimal code fragments, etc. Reviewers can also suggest improvements that involve code efficiency and complexity, software libraries, best practices, refactoring, code quality, code optimization, documentation, etc. The identified issues and improvements are expressed by means of comments. The comments may be descriptive where the issues are detailed. However, comments may also be actionable where the reviewers recommend solutions to fix the issues. 
Code review comments are very useful as they enable developers, \ie authors of the code changes, to get feedback from experienced developers. This leads to better collaboration, communication, and knowledge-sharing within a team while maintaining a good codebase quality. This helps also avoid technical debt, which refers to the additional cost and effort required to fix issues that are not caught early in the development process.
Automating code review comments generation can bring several benefits to the software development process. 
Firstly, it can help save time and effort by reducing the amount of manual work needed to review and provide feedback on code. This enables teams to move faster in their development process.
The automation of this process helps to produce objective feedback without being influenced by personal preferences, relationships, health, well-being, etc.


\paragraph*{\textbf{Code refinement}}
The comments that are produced by the previous step are fed as input to the code refinement phase. The developers, and authors of the code changes, should consider the feedback of the reviewers and perform the necessary code changes. Developers should solve the issues described in the comments or apply suggested solutions. New code changes are pushed again to the project repository and should satisfy the reviewer's comments. The refined version of the source code is examined again by the reviewers to check whether the comments are properly addressed. Proper code refinement requires a good understanding of the reviewer's comments. That is, the reviews provided should be clear, specific, and comprehensible.



\subsection{Pre-trained language models}

In recent years, the Natural Language Processing (NLP) domain has dramatically evolved. 
State-of-the-art language models, that are based on the transformer architecture \cite{vaswani2017attention}, have shown outstanding performance in solving natural language problems.
Transformers have several advantages over recurrent neural networks. They enable parallel computations which reduces training time and captures long-range dependencies efficiently.
\emph{BERT}\cite{devlin2018bert}, \emph{GPT-3}\cite{radford2019language}, \emph{XLNet} \cite{yang2019xlnet}, \emph{RoBERTa} \cite{liu2019roberta} and \emph{T5} \cite{raffel2019exploring} are examples of general-purpose transformers that were pre-trained on tons of data to provide general and high-level representations of text.
\emph{CodeBERT} \cite{feng2020codebert} and \emph{CodeT5} \cite{wang2021codet5} are examples of transformers that were pre-trained on source code data.
These pre-trained models could then be adapted (\ie fine-tuned) on downstream tasks using specific datasets (\eg fine-tune a language model to predict if a code fragment contains bugs).

% transformer architecture and how it works
Transformers are sequence-to-sequence models based on the attention mechanism that takes into account the relationship between all the words in the sentence and not only the contextual words (\eg previous and next words).
The attention mechanism learns a weighting function indicating how much each element contributes to the prediction (\ie importance of each input element in predicting the target). 
A transformer is composed of encoders and decoders.
The encoder transforms the input sequence into contextual embeddings. 
These latter encode the meaning of each word of the input based on its context in low-dimension and high-level representations.
The decoder uses these contextual representations to predict the output sequence.

\emph{CodeT5} \cite{wang2021codet5} is a pre-trained encoder-decoder transformer for code that is pre-trained on $8.35M$ functions in 8 programming languages.
There are several versions of \emph{codeT5}. The small version has $60$ million parameters and the base version has $220$ million parameters.





\subsection{Knowledge distillation}
\label{Sec:distillation}
% $\mathcal{D} = {(x_i, y_i)}_{i=1}^{n}$
Knowledge distillation is a popular technique that was first introduced by Hinton et al. \cite{hinton2015distilling} as a method to transfer knowledge from a complex model, also known as the teacher, to a smaller and faster model, called the student. The main goal of knowledge distillation is to transfer the learned knowledge of the teacher model to the student model so that it can achieve comparable or even better performance on a target task.

The process of knowledge distillation consists of training a teacher model on a large dataset to accomplish a specific task. Then, the student model is trained to mimic the behavior of the teacher model by minimizing the distance between their output distributions on the same dataset, typically using the Kullback-Leibler divergence (KL-divergence) as the distance metric \cite{joyce2011kullback, kim2021comparing}.

For instance, this concept is employed in model compression where the knowledge is transferred from a large and complex neural network (\ie the teacher) to a smaller and simpler neural network (\ie the student). The goal of knowledge distillation is to make the student network learn the same function as the teacher network but with fewer parameters. 

Cross-task knowledge distillation is a recent extension of knowledge distillation that enables the transfer of knowledge from one task to another\cite{ye2020distilling, yuan2019ckd, yang2022cross, li2022prototype}. Instead of transferring knowledge from a complex model to a smaller one for the same task, cross-task knowledge distillation transfers knowledge from a model trained on one task, referred to as the source task, to a model trained on a different task, referred to as the target task. This allows the target model to improve its performance, even if the two tasks are not directly related.





